When does a predictor know its own loss?

Given a predictor and a loss function, how well can we predict the loss that the predictor will incur on an input? This is the problem of loss prediction, a key computational task associated with uncertainty estimation for a predictor. In a classification setting, a predictor will typically predict a distribution over labels and hence have its own estimate of the loss that it will incur, given by the entropy of the predicted distribution. Should we trust this estimate? In other words, when does the predictor know what it knows and what it does not know? In this work we study the theoretical foundations of loss prediction. Our main contribution is to establish tight connections between nontrivial loss prediction and certain forms of multicalibration, a multigroup fairness notion that asks for calibrated predictions across computationally identifiable subgroups. Formally, we show that a loss predictor that is able to improve on the self-estimate of a predictor yields a witness to a failure of multicalibration, and vice versa. This has the implication that nontrivial loss prediction is in effect no easier or harder than auditing for multicalibration. We support our theoretical results with experiments that show a robust positive correlation between the multicalibration error of a predictor and the efficacy of training a loss predictor.

==> macros-old.tex <==
\usepackage[utf8]{inputenc}
\usepackage{amsmath, amssymb,amsfonts, amsthm, bbm, graphicx, url, hyperref, cleveref, setspace}
\renewcommand\qedsymbol{$\blacksquare$}
\hypersetup{colorlinks}
\usepackage{float}
\usepackage{graphicx}
\usepackage{bm}
\usepackage{amssymb}
\usepackage{bbm}
\usepackage{xcolor}
\usepackage{algorithm}
\usepackage{dsfont}
\usepackage{xspace}
\usepackage{comment}
\usepackage{tikz}
\usepackage{dsfont}
\usepackage{fullpage}

\newcommand{\eat}[1]{}

\newcommand{\addtag}{\addtocounter{equation}{1}\tag{\theequation}}
\newcommand{\omnip}{{\bf Omniprediction}}
\newcommand{\op}{\mathrm{OP}}
\newcommand{\innerp}{{\bf Inner Production}}
\newcommand{\ip}{\mathrm{IP}}
\newcommand{\expest}{{\bf Expectation Estimation}}
\newcommand{\ee}{\mathrm{EE}}
\newcommand{\iprod}[2]{{\langle #1, #2 \rangle}}
\newcommand{\Integ}{d^{-1}}
\newcommand{\diff}[1]{\mD^{(#1)}}
\newcommand{\df}{\mathrm{diff}}
\newcommand{\cross}{\mathrm{cross}}
\newcommand{\coll}{\mathrm{coll}}


\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\mC}{\mathcal{C}}
\newcommand{\mD}{\mathcal{D}}
\newcommand{\mE}{\mathcal{E}}
\newcommand{\mA}{\mathcal{A}}


\newcommand{\mU}{\mathcal{U}}
\newcommand{\mH}{\mathcal{H}}
\newcommand{\mS}{\mathcal{S}}
\newcommand{\mT}{\mathcal{T}}
\newcommand{\mA}{\mathcal{A}}
\newcommand{\mB}{\mathcal{B}}
\newcommand{\mF}{\mathcal{F}}
\newcommand{\mG}{\mathcal{G}}
\newcommand{\mI}{\mathcal{I}}
\newcommand{\mL}{\mathcal{L}}
\newcommand{\mM}{\mathcal{M}}
\newcommand{\grad}{\nabla}
\newcommand{\dist}{\mathrm{ExpDist}}
\newcommand{\Dzo}{\Delta_{[0,1]}}
 

\newcommand{\mLC}{\mathcal{L}_\mathsf{cvx}}
\newcommand{\mFC}{\mathcal{F}_\mathsf{cvx}}
\newcommand{\ex}{\mathrm{ex}}

\newcommand{\mW}{\mathcal{W}}
\newcommand{\mX}{\mathcal{X}}
\newcommand{\mP}{\mathcal{P}}
\newcommand{\mQ}{\mathcal{Q}}

\newcommand{\mcal}{\mathrm{MC}}
\newcommand{\mcals}{\mathrm{MC}^\mathrm{s}}
\newcommand{\mcalreg}{\mathrm{MC}^\mathrm{f}}
\newcommand{\macc}{\mathrm{MA}}
\newcommand{\Bad}{\mathrm{Bad}}
\newcommand{\relu}{\mathrm{ReLU}}

\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\Bin}{Bin}
\renewcommand{\Im}{\mathrm{Im}}

\newcommand{\tf}{\tilde{p}}
\newcommand{\tp}{\tilde{p}}
\newcommand{\ty}{\mathbf{\tilde{y}}}


\newcommand{\Q}{{\mathbb{Q}}}
\newcommand{\R}{{\mathbb{R}}}
\newcommand{\Z}{{\mathbb{Z}}}
\newcommand{\N}{{\mathbb{N}}}
\newcommand{\F}{{\mathbb{F}}}


\newcommand{\mFS}{\mathcal{F}^\mathcal{S}}

\newcommand{\hy}{\hat{y}}
\newcommand{\bll}{\bar{\ell}}

\newcommand{\mb}[1]{\mathbf{#1}}

\renewcommand{\d}{\mathrm{d}}
\renewcommand{\i}{\mathbf{i}}
\renewcommand{\j}{\mathbf{j}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\sy}{\mathbf{y^*}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bt}{\mathbf{t}}


\newcommand{\x}{\mathbf{x}}
\newcommand{\z}{\mathbf{z}}
\newcommand{\s}{\mathbf{S}}

\newcommand{\logf}[2]{\ensuremath{\log\left(\frac{#1}{#2}\right)}}
\newcommand{\rgta}{\rightarrow}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\RHS}{\mathrm{RHS}}
\newcommand{\LHS}{\mathrm{LHS}}
\newcommand{\lt}{\left}
\newcommand{\rt}{\right}


\newcommand{\zo}{\ensuremath{\{0,1\}}}
\newcommand{\izo}{\ensuremath{[0,1]}}

\newcommand{\ren}[3]{D_{#1}\big( #2 \| #3 \big)}
\newcommand{\dtv}{\mathrm{d_{TV}}}
\newcommand{\qme}{\ensuremath{Q^{\mathrm{ME}}}}
\newcommand{\wme}{\ensuremath{w^{\mathrm{ME}}}}


\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\onenorm}[1]{\left\lVert#1\right\rVert_1}
\newcommand{\infnorm}[1]{\left\lVert#1\right\rVert_\infty}
\newcommand{\normfr}[1]{\left\lVert#1\right\rVert_{\text{F}}}
\newcommand{\llv}{\left\lvert}
\newcommand{\rrv}{\right\rvert}
\newcommand{\fD}{\mathcal{D}_{\tp}}
\newcommand{\Dv}{{\mathcal{D}|_{\bv}}}
\newcommand{\tD}{\mathcal{D}_f}



\newcommand{\ellc}{\ell_{\mathsf{cor}}}
\newcommand{\Pell}{\partial \ell}


\newcommand{\OI}{Outcome Indistinguishability\xspace}
\newcommand{\Oi}{Outcome indistinguishability\xspace}
\newcommand{\oi}{outcome indistinguishability\xspace}

\newcommand{\OIble}{Outcome Indistinguishable\xspace}
\newcommand{\Oible}{Outcome indistinguishable\xspace}
\newcommand{\oible}{outcome indistinguishable\xspace}


\newcommand{\Macc}{Multiaccuracy\xspace}
\newcommand{\mact}{multiaccurate\xspace}
\newcommand{\Mcab}{Multicalibration\xspace}
\newcommand{\mcab}{multicalibration\xspace}
\newcommand{\mcbd}{multicalibrated\xspace}
\newcommand{\mcbn}{approximate multicalibration\xspace}
\newcommand{\Mcbn}{Approximate multicalibration\xspace}
\newcommand{\smcbd}{multicalibrated\xspace}
\newcommand{\maxent}{MaxEnt}
\newcommand{\B}[1]{\mathrm{Ber(#1)}}
\newcommand{\Hspc}{\mathrm{Thr_{\mathcal{C}}}}
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\pdf}{\mathrm{D}}
\newcommand{\mrF}{\mathrm{F}}
\newcommand{\mrG}{\mathrm{G}}
\newcommand{\mrA}{\mathrm{A}}
\newcommand{\mrB}{\mathrm{B}}


\newcommand{\Deltak}{\Delta_{[k]}}


\newcommand{\eps}{\varepsilon}
\newcommand{\lsq}{\ensuremath{\left[}}
\newcommand{\rsq}{\ensuremath{\right]}}
\newcommand{\lb}{\ensuremath{\left(}}
\newcommand{\rb}{\ensuremath{\right)}}
\newcommand{\abs}[1]{\ensuremath \Bigl\lvert #1 \Bigr\rvert}
\newcommand{\lst}{\ensuremath{\left|}}
\newcommand{\rst}{\ensuremath{\right|}}
\newcommand{\lam}{\ensuremath{\lambda}}
\newcommand{\la}{\ensuremath{\langle}}
\newcommand{\ra}{\ensuremath{\rangle}}



\newcommand{\pmo}{\ensuremath{ \{\pm 1\} }}
\newcommand{\fr}[1]{\ensuremath{\frac{1}{#1}}}
\newcommand{\fp}[2]{\ensuremath{\frac{\partial #1}{\partial #2}}}
\newcommand{\lexp}{\ensuremath{\ell_{\exp}}}
\newcommand{\llgt}{\ensuremath{\ell_{\mathrm{lgt}}}}
\newcommand{\sD}{\ensuremath{(\x, \y) \sim \D}}
\newcommand{\err}{\mathrm{err}}
\newcommand{\opt}{\mathrm{OPT}}
\newcommand{\ind}[1]{\ensuremath{\mathbbm{1}(#1)}}
\newcommand{\dtsim}{\mathrm{D}^{||}}
\newcommand{\rdsim}{\mathrm{R}^{||}}
\newcommand{\dtow}{\mathrm{D}^{1}}
\newcommand{\rdow}{\mathrm{R}^{1}}
\newcommand{\dt}{\mathrm{D}}
\newcommand{\rd}{\mathrm{R}}
\newcommand{\gh}{\mathrm{gapH}}
\newcommand{\samp}{\leftarrow}
\newcommand{\indx}{\mathrm{Index}}
\newcommand{\ab}{\mathrm{Abs}}



\newcommand{\defeq}{{:=}}
\DeclareMathOperator*{\cor}{{\bf {cor}}}
\DeclareMathOperator*{\SD}{{\bf {SD}}}
\DeclareMathOperator*{\Sup}{{\bf {Sup}}}
\newcommand{\C}{\mathcal{C}}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\poly}{poly}
\DeclareMathOperator{\nnz}{nnz}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\new}{new}
\DeclareMathOperator{\pre}{pre}
\DeclareMathOperator{\old}{old}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\T}{\top}
\DeclareMathOperator*{\E}{\mathbf{E}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\clip}{clip}
\DeclareMathOperator{\Lin}{Lin}
\newcommand{\Ber}{\mathrm{Ber}}
\newcommand{\Lip}[1]{\mathcal{L}_{#1}}

\newcommand{\etal}{{\it et al.}}
\newcommand{\MS}[1]{{\color{blue}[Mihir: #1]}}
\newcommand{\UW}[1]{{\color{green}[Udi: #1]}}
\newcommand{\PG}[1]{{\color{red}[Parikshit: #1]}}
\newcommand{\mpk}[1]{{\color{violet} [mpk: #1]}}


\newcommand{\todo}[1]{{\color{red} [\textbf{TODO:} #1]}}


\newcommand{\note}[1]{{\textcolor{red}{~{\textbf{\emph{[#1]}}}}~}}
\newcommand{\sign}{\mathrm{sign}}
\newcommand{\sj}[1]{{\color{blue} [SJ: #1]}}

\newcommand{\bE}{{\mathbb{E}}}



\newcommand{\card}[1] {\left\vert #1 \right\vert}
\newcommand{\set}[1] {\left\{ #1 \right\}}
\newcommand{\given}{~\middle \vert~}
\newcommand{\lr}[1]{\left[~ #1 ~\right]}



\newcommand{\ft}{\tilde{f}}
\newcommand{\fs}{f^*}
\newcommand{\VC}{\mathsf{VC}}
\newcommand{\mce}{\mathsf{MCE}}
\newcommand{\umce}{\mathsf{sMCE}}
\newcommand{\smce}{\mathsf{sMCE}}
\newcommand{\ce}{\mathsf{CE}}
\newcommand{\lglm}{\mathcal{L}_\mathsf{GLM}}









\newtheorem{result}{Theorem} %
\newtheorem{minorresult}[result]{Proposition}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{notation}[theorem]{Notation}

\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{example}[theorem]{Example}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{open}[theorem]{Open Problem}

\newcommand{\cR}{\mathsf{R}}
\newcommand{\cD}{\mathsf{D}}


==> preliminaries.tex <==
We consider a binary prediction task over a space $\calX$. Given some true unknown distribution $\calD$ over $\calX \times \{0, 1\}$, we denote $\pbayes(x) := \mathbb{E}_{\calD}[y|x]$ as the true conditional distribution of $y$ given each $x$. We assume that we are provided some pre-trained predictor $\pred: \calX \rightarrow [0, 1]$. 

\subsection{Losses and the Discrete Derivative}
A loss function $\ell: \{0, 1\} \times [0, 1] \rightarrow \R_{\geq 0}$ gives a measure of the loss suffered when we predict some value in $[0, 1]$ compared to the true label. Define the expected loss $L : [0, 1] \times [0, 1] \to \R_{\geq 0}$ at $x \in \calX$ to be $L \divx{\pbayes(x)}{\pred(x)} = \ex_{y \sim \Ber(\pbayes(x))}[\ell(y, \pred(x))]$. 

We note the following useful fact: 
\begin{fact}\label{fact:loss-def}
    For any loss $\ell: \{0, 1\} \times [0, 1] \rightarrow \R$, and $v \in [0, 1]$ we have that $\ell(y, v)$ can be equivalently rewritten as 
    \[\ell(y, v) = y(\ell(1, v) - \ell(0, v)) + \ell(0, v).\]    
\end{fact}

For ease of notation, given a loss $\ell$ and $v \in [0, 1]$, we will denote the ``discrete derivative" of $\ell$ at $v$ as 
\[\delta_{\ell}(v) := \ell(1, v) - \ell(0, v).\] 


For any loss $\ell$, if the labels are drawn according to $y \sim \Ber(\pbayes(x))$ for any $\pbayes(x) \in [0, 1]$, then the optimal prediction that minimizes the loss, $k_{\ell}(\pbayes(x)) \in [0, 1]$ is defined by 
\[k_{\ell}(\pbayes(x)) = \argmin_{v \in [0, 1]}\ex_{y \sim \Ber(\pbayes(x))}[\ell(y, v)] = \argmin_{v \in [0, 1]}L\divx{\pbayes(x)}{v}.\]



We call the loss \emph{proper} if for all $\pbayes(x) \in [0, 1]$, it is minimized by predicting $\pbayes(x)$, i.e. 
\[L\divx{\pbayes(x)}{\pbayes(x)} = L\divx{\pbayes(x)}{k_{\ell}(\pbayes(x))}.\]

Notable examples of proper losses include the square loss and cross entropy loss. An example of a non-proper loss is the $\ell_1$-loss, $\ell_1(y, v) = |y - v|$. In this case, the optimal prediction is obtained by rounding $\pbayes(x)$ to the nearest value in $\{0, 1\}$. 

We note that composing any loss $\ell$ with its associated optimal post-processing function $k_{\ell}$ results in a proper loss, even if $\ell$ itself is non-proper. In particular, let $\ell_k(y, v) = \ell(y, k_{\ell}(v))$ for any loss $\ell$. Then, we have that for any point $x \in \calX$,
\begin{align*}
    L_k\divx{\pbayes(x)}{\pbayes(x)} &= \ex_{y \sim \Ber(\pbayes(x))}[\ell_k(y, \pbayes(x))]\\
    &= \ex_{y \sim \Ber(\pbayes(x))}[\ell(y, k_{\ell}(\pbayes(x)))]\\
    &= \ex_{y \sim \Ber(\pbayes(x))}[\ell(y, \argmin_{v \in [0, 1]}\ex_{y \sim \Ber(\pbayes(x))}[\ell(y, v)])]\\
    &= \min_{v \in [0, 1]}\ex_{y \sim \Ber(\pbayes(x))}[\ell(y, v)]\\
    &= \min_{v \in [0, 1]}\ex_{y \sim \Ber(\pbayes(x))}[\ell(y, k_{\ell}(v))]\\
    &= L_k\divx{\pbayes(x)}{k_{\ell_k}(\pbayes(x))}
\end{align*}
implying that $\ell_k$ is indeed proper. Thus, we can extend any discussion of proper losses to include non-proper losses when predictions are made using the optimal post-processed value. 

Define the generalized entropy function $H(v) = L \divx{v}{v}$, and the generalized (Bregman) divergence $D \divx{\pbayes(x)}{v} = L \divx{\pbayes(x)}{v} - H(\pbayes(x))$.

In the case of proper losses, prior works have noted an important characterization of proper losses with respect to their associated concave generalized entropy functions $H_{\ell}(v)$ \cite{gneiting2007strictly, kleinberg2023u}. In particular, every concave function $H: [0, 1] \rightarrow \R_{\geq 0}$ gives rise to a proper loss $\ell$ defined by 
\[\ell(1, v) = H(v) + (1 - v)H'(v)\]
\[\ell(0, v) = H(v) - v H'(v) \]
where $H'(v)$ is a ``superderivative'' of $H$, i.e. for any $v, w \in [0, 1]$, $H(v) \leq H(w) + (v - w)H'(w)$. When $H(v)$ is differentiable at all $v \in [0, 1]$, the superderivative is unique, and is just the derivative. 

In the reverse direction, any proper loss (with some regularity assumptions) has the above form for the concave function $H(v) = L\divx{v}{v}.$

Thus, we get the following characterization of the discrete derivative $\delta_{\ell}$:
\begin{proposition}
    For any proper loss $\ell$ defined by a differentiable concave function $H_{\ell}:[0,1] \rightarrow \R_{\geq 0}$, we have that for all $v \in [0,1],$
\begin{align*}
    \delta_{\ell}(v) = H'_{\ell}(v)
\end{align*}
\end{proposition}

\begin{proof}
    The statement follows immediately from the above fact and definition of $\ell$ in terms of its concave entropy function:
    \begin{align*}
    \delta_{\ell}(v) &= \ell(1, v) - \ell(0,v) \\
    &= H_{\ell}(v) + (1-v)H'_{\ell}(v) - (H_{\ell}(v) - \pred H'_{\ell}(v))\\
    &= H'_{\ell}(v).
\end{align*}
    
\end{proof}

In other words, when $\ell$ is a proper loss, $\delta_{\ell}(v)$ is just the derivative of $\ell$'s generalized entropy function at $v$. 
\todo{Notation ($v$, $\pred$, $\pbayes$).}

\subsection{Loss Predictors and the Self-Entropy Predictor}

Given a predictor $p: \calX \rightarrow [0,1]$ and a proper loss $\ell: \{0,1\} \times [0,1] \rightarrow \R_{\geq}$, a \emph{loss predictor} for $\ell$ and $p$, $\lossPred: \calX \times [0,1] \rightarrow \R_{\geq 0}$, provides point-wise estimates $\lossPred(x, p(x))$ of the loss at each $x \in \calX$. 

\todo{exact format for loss predictor needs to be ironed out (notation, does it get additional features, etc) }

A perfect loss-predictor would predict exactly the true expected loss at each $x$, i.e. $\lossPred(x, p(x)) = L\divx{\pbayes(x)}{\pred(x)}$. 
\todo{introduce square loss as a natural objective}

In the absence of any other information or data, $\pred$ itself can be used to construct loss predictions, which we refer to as the \emph{self-entropy predictor.} In particular, if we believe $\pred$ to be close to $\pbayes$, then a natural estimate of the loss at a particular point $x$ would be the loss incurred if $\pbayes(x) = \pred(x)$, i.e. $L\divx{\pred(x)}{\pred(x)} = H_{\ell}(\pred(x))$. 

\begin{definition}[Self-Entropy Predictor]
    Given a proper loss $\ell$ and predictor $\pred$, we define the \emph{self-entropy predictor} for $\ell$ and $p$ to be the predictor that outputs $\ell$'s generalized entropy value for each prediction:
    \[\lossPred(x, \pred(x)) = H_{\ell}(\pred(x)).\]
\end{definition}

This definition of the self-entropy predictor is not arbitrary. In particular, we can show that when $\pred$ is calibrated, it is the optimal post-processing of $\pred$'s predictions to produce a loss predictor. 
\todo{need to define calibration before this, or put later}

\begin{lemma}\label{lem:self-entropy-opt}
    Consider any proper loss $\ell$ and calibrated predictor $p$. Then, 

    \[H_{\ell} = \argmin_{G: [0,1] \rightarrow \R_{\geq 0}} \ex_{x \sim \calD_{\calX}}[(L\divx{\pbayes(x)}{\pred(x)} - G(\pred(x)))^2].\]
    I.e., among all possible post-processings of the predictor $\pred$ to produce a loss predictor, $H_{\ell}$ is the one that minimizes the square loss of the resulting loss predictor.
\end{lemma}

\begin{proof}[Proof sketch]
We sketch a proof that the self-entropy is the best loss predictor purely as a function of the prediction (and not the point) if the predictor is calibrated --- i.e. the best loss predictor that is constant on the level sets.

Consider a single level set $[x]$ where we predict $p(z) = p$ for all $z \in [x]$. The self-entropy loss prediction on this entire level set is $H(p)$.

Let the level set consist of $n$ points $z_1, \dots, z_n$, with true probabilities $\pbayes(z_1), \dots, \pbayes(z_n)$. And the true losses wrt the prediction $p$ are $L^*_i := L \divx{\pbayes(z_i)}{p}$.

Now what is the optimal constant loss prediction on this level set? If we mean optimal in terms of having least expected square loss wrt the true $L^*_i$, i.e. $\arg \min \ex_i (L - L^*_i)^2$, then the optimum is precisely the mean, $L = \ex_i [L^*_i]$.

Now miraculously by linearity of expectation, \begin{align*}
    \ex_i [L^*_i] &= \ex_{z_i \sim [x]} [L \divx{\pbayes(z_i)}{p}] \\
    &= \ex_{z_i \sim [x]} \ex_{y \sim \pbayes(z_i)} \ell(y, p) \\
    &= L \divx{\ex_{z_i \sim [x]} \pbayes(z_i)}{p} \\
    &= L \divx{p}{p} \\
    &= H(p),
\end{align*} proving optimality. Basically we can send the expectation in because $L$ is linear in the first argument (i.e.\ the truth), and then use the key fact that $\ex_{z_i \sim [x]} \pbayes(z_i) = p$ since the predictor is calibrated.

In fact I think this proof also establishes the converse, i.e.\ if the self-entropy loss prediction is optimal it can only be because we are calibrated on that level set.
\end{proof}

It turns out that the performance of the self-entropy predictor is highly connected to the closeness of $\pbayes$ and $\pred$ as well as the discrete derivative of the loss in question. 

\begin{lemma}[Pointwise Loss Gap]
    Given any proper loss $\ell$ and predictor $p$, the point-wise distance between the true loss and self-entropy prediction for any $x \in \calX$ can be equivalently expressed as 
    \[L\divx{\pbayes(x)}{\pred(x)} - H_{\ell}(\pred(x)) = (\pbayes(x) - \pred(x))\delta_{\ell}(\pred(x)).\]
\end{lemma}
In other words, the quality of the self-entropy predictor can be connected to a re-weighted version of the quality of $\pred$ itself. 

\begin{proof}
    We have 
    \begin{align*}
    L\divx{\pbayes(x)}{\pred(x)} - H_{\ell}(\pred(x)) &= \ex_{y \sim \Ber(\pbayes(x))}\ex[\ell(y, \pred(x))] - \ex_{\tilde y \sim \Ber(\pred(x))}\ex[\ell(\tilde y, \pred(x))]\\
    &= \pbayes\delta_{\ell}(\pred(x)) + \ell(0,\pred(x)) - (\pred(x)\delta_{\ell}(\pred(x)) + \ell(0, \pred(x))) \tag{Fact~\ref{fact:loss-def}}\\
    &= (\pbayes(x) - \pred(x))\delta_{\ell}(\pred(x))
    \end{align*}
\end{proof}

This relationship will prove crucial for linking the accuracy of loss prediction to the multicalibration of the pre-trained predictor. We next introduce and define multicalibration. 

\subsection{Multicalibration}


==> training.tex <==
\section{Loss Predictor Training Details}
\label{sec:training}

